Private Language Models via Truncated Laplacian Mechanism

Deep learning models for NLP tasks are prone to variants of privacy attacks. To prevent privacy leakage, researchers have investigated word-level perturbations, relying on the formal guarantees of differential privacy (DP) in the embedding space. However, many existing approaches either achieve unsatisfactory performance in the high privacy regime when using the Laplacian or Gaussian mechanism, or resort to weaker relaxations of DP that are inferior to the canonical DP in terms of privacy strength. This raises the question of whether a new method for private word embedding can be designed to overcome these limitations. In this paper, we propose a novel private embedding method called the high dimensional truncated Laplacian mechanism. Specifically, we introduce a non-trivial extension of the truncated Laplacian mechanism, which was previously only investigated in one-dimensional space cases. Theoretically, we show that our method has a lower variance compared to the previous private word embedding methods. To further validate its effectiveness, we conduct comprehensive experiments on private embedding and downstream tasks using three datasets. Remarkably, even in the high privacy regime, our approach only incurs a slight decrease in utility compared to the non-private scenario.

==> tab/tab10.tex <==
\begin{table*}[htbp]
\caption{Performance of GloVe Embedding with non-privacy protection (i.e., the privacy budget is infinite) and with three mechanisms (Gussian, Laplacian and TrLaplacian), the  privacy budget ranges from 5 to 50.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccccccccc}
\toprule 
 &  & \textbf{Original} &  & \multicolumn{4}{c}{\textbf{Guassian}} &  & \multicolumn{4}{c}{\textbf{Laplacian}} &  & \multicolumn{4}{c}{\textbf{TrLaplacian}} \\ \cmidrule{3-3} \cmidrule{5-8} \cmidrule{10-13} \cmidrule{15-18} 
\textbf{Privacy budget $\bm{\epsilon}$} &  & $\infty$ &  & 1     & 5    & 10    & 20    &  & 1     & 5    & 10    & 20    &  & 1              & 5    & 10    & 20    \\ \midrule
\textbf{Yahoo}:           &  &                          &  &       &       &       &       &  &       &       &       &       &  &                &       &       &       \\
\rowcolor{lightgray}
accuracy             &  &   2.95  &  & 4.28  & 3.01  & 3.03  & 2.98  &  & 4.93  & 3.24  & 3.05  & 3.13  &  & \textbf{2.85}  & \textbf{2.97}  &  \textbf{2.92} & \textbf{2.81}  \\
\rowcolor{lightgray}
Rouge1           &  &      (92.24/92.52)               &  & (90.85/91.12) & (92.16/92.41) & (92.05/92.29)  & (92.08/92.33) &  & (89.79/90.29) & (91.95/92.25) & (92.12/92.47) & (92.11/92.43) &  & (92.31/92.54) & (92.18/92.55) & (92.13/92.38) & (92.36/92.56) \\
\rowcolor{lightgray}
BLEU             &  &                     &  &  &   &  &  &  &  &    &  &  &  &         &  &  &  \\ 
\midrule
\textbf{Yelp}:            &  &                          &  &       &       &       &       &  &       &       &       &       &  &                &       &       &       \\
Loss             &  &  3.07                    &  &  4.74 & 3.14  & 3.13  & 2.97  &  & 5.02  & 3.30  & 3.66   & 3.17  &  & \textbf{2.93}  & \textbf{3.03}  & \textbf{3.00}  & \textbf{2.98}  \\
Rouge1           &  &      (89.13/89.74) &  & (86.25/87.08) & (88.86/89.47) & (88.97/89.63) & (89.45/90.23) &  & (86.13/86.80) & (88.77/89.38) & (87.87/88.51) & (88.97/89.56) &  & (89.37/90.06) &  (89.19/89.67) & (89.08/89.74) & (89.34/89.93)\\
BLEU             &  &                    &  &   &  &  &  &  &  &  &   &  &  &     &  &  &  \\ 
\bottomrule
\end{tabular}%
}
\end{table*}



accuracy:

non-pri: 89.70

e=1
gau:89.54 lap:89.54, trlap: 90.01



epoch: 50
batch size = 1024
learning rate = 0.0005

C = 0.005



\begin{table*}[!htbp]
\caption{\textbf{Privacy.} Performance of GloVe Embedding with non-privacy protection (i.e., the privacy budget is infinite) and with three mechanisms (Gaussian, Laplacian and TrLaplacian), the  privacy budget ranges from 1 to 20. $\uparrow$ means a higher value under this metric indicates better results, and $\downarrow$ means the opposite. The best performance is \textbf{bolded}. \label{tb:1}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccccccccc}
\toprule 
 & &  & \textbf{Original} &  & \multicolumn{4}{c}{\textbf{Gaussian}} &  & \multicolumn{4}{c}{\textbf{Laplacian}} &  & \multicolumn{4}{c}{\textbf{TrLaplacian}} \\ \cmidrule{4-4} \cmidrule{6-9} \cmidrule{11-14} \cmidrule{16-19} 
\multicolumn{2}{c}{\textbf{Privacy budget $\bm{\epsilon}$}} &  & $\infty$ &  & 1     & 5    & 10    & 20    &  & 1     & 5    & 10    & 20    &  & 1              & 5    & 10    & 20    \\ 
\midrule
\rowcolor{lightgray}
\multirow{4}{*}{\textbf{Yahoo}} & \textbf{Loss\bm{$\downarrow$}}             &  &   2.95  &  & 4.28  & 3.01  & 3.03  & 2.98  &  & 4.93  & 3.24  & 3.05  & 3.13  &  & \textbf{2.85}  & \textbf{2.97}  &  \textbf{2.92} & \textbf{2.81}  \\
& \textbf{Rouge1\bm{$\uparrow$}}           &  &    92.37  &  & 90.97 & 92.27 & 92.16  & 92.19 &  & 90.02 & 92.09 & \textbf{92.28} & 92.26 &  & \textbf{92.41} &  \textbf{92.35} & 92.24 & \textbf{92.45} \\
& \textbf{BLEU\bm{$\uparrow$}}             &  &  8.501  &  & 8.501 & 8.501  & 8.499 & \textbf{8.500} &  & \textbf{8.503} &  8.501  & \textbf{8.502} & 8.500 &  & 8.498  & \textbf{8.501} & 8.499 & 8.499 \\
\rowcolor{lightgray}
& \bm{$N_w\uparrow$}             &  & 0.703 &  &  0.637 & 0.680 & 0.664 & 0.672 &  & 0.660 & 0.658 & 0.675  & 0.655 &  &  \textbf{0.674}  & \textbf{0.670} & \textbf{0.702} & \textbf{0.680} \\
\midrule
\rowcolor{lightgray}
\multirow{4}{*}{\textbf{Yelp}} & \textbf{Loss\bm{$\downarrow$}}             &  &  3.07                    &  &  4.74 & 3.14  & 3.13  & 2.97  &  & 5.02  & 3.30  & 3.66   & 3.17  &  & \textbf{2.93}  & \textbf{3.03}  & \textbf{3.00}  & \textbf{2.98}  \\
& \textbf{Rouge1\bm{$\uparrow$}}           &  &   89.40  &  & 86.63 & 89.13 & 89.27 & \textbf{89.80} &  & 86.43 & 89.04 & 88.15 & 89.23 &  & \textbf{89.68} & \textbf{89.40}  & \textbf{89.37} & 89.60 \\
& \textbf{BLEU\bm{$\uparrow$}}             &  & 8.934 &  &  8.933 & \textbf{8.936} & 8.933 & \textbf{8.944} &  & 8.931 & 8.932 & 8.933  & 8.934 &  &  \textbf{8.934}  & 8.931 & \textbf{8.934} & 8.938 \\
\rowcolor{lightgray}
& \bm{$N_w\uparrow$}     &  & 0.706 &  &  0.708 & \textbf{0.725} & 0.708 & 0.739 &  & 0.691 & 0.721 & 0.704  & 0.699 &  &  \textbf{0.724} & 0.700 & \textbf{0.712} & \textbf{0.740} \\
\bottomrule
\end{tabular}%
}
\end{table*}




Yelp:
--0.05
gau: (15.98/16.04)
lap: (12.57/12.82)
trlap: (89.23/89.73)

--0.1
gau: (48.72/49.16)
lap: (14.70/14.73)
trlap: (89.23/89.79)

--0.2
gau: (76.20/76.85)
lap: (66.31/67.04)
trlap: (89.06/89.69)

--0.5
gau: (84.66/85.37)
lap: (81.89/82.34)
trlap: (89.29/89.86)


Yahoo:
--0.05
gau: (14.09/14.04)
lap: (13.32/12.84)
trlap: (92.31/92.60)


--0.1
gau: (59.10/60.06)
lap: (42.65/44.27)
trlap: (92.31/92.57)


--0.2
gau: (83.41/83.86)
lap: (75.44/76.17)
trlap: (92.30/92.54)


--0.5
gau: (88.91/89.25)
lap: (86.89/87.12)
trlap: (92.10/92.43)



==> tab/tab2.tex <==
% \begin{table*}[!htbp]
% \caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) for different mechanisms under various privacy budget via sentiment analysis task over the IMDB dataset.\label{tb:2}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clccclccclccc}
% \toprule
%  &  & \multicolumn{3}{c}{\textbf{Random(seed = 42)}}           &  & \multicolumn{3}{c}{\textbf{GloVe}}                    &  & \multicolumn{3}{c}{\textbf{fastText}}                 
% \\ \cline{3-5} \cline{7-9} \cline{11-13} 
% \textbf{Privacy budget $\bm{\epsilon}$}         &  
% & TrLaplace       & Laplace & Guassian &  
% & TrLaplace       & Laplace         & Guassian &  
% & TrLaplace       & Laplace         & Guassian \\ \midrule
% $\bm{0.05}$       &  
% &\textbf{87.12}  &  84.24 &  85.47  &  
% & \textbf{87.18} &     86.77      &  87.11  &  
% & \textbf{87.40} &   87.38        & 87.29  \\
% \rowcolor{lightgray}
% $\bm{0.1}$     &  
% & 85.52 & \textbf{85.94} & 85.59  & 
%      &  86.54 
% &  84.52 &  \textbf{86.73}  &   
% &\textbf{87.80} &   86.74        & 87.15  \\
% $\bm{0.2}$    &   
% & 87.04 &  86.93  &\textbf{87.07}    & 
%  & 86.95 &  \textbf{87.07}      &   84.27 &  
% &    \textbf{86.94}      & 86.44 &  86.60  \\
% \rowcolor{lightgray}
% $\bm{0.5}$     & 
%  &  \textbf{87.29} &  86.71 & 86.65     & 
%  &        \textbf{87.33}   & 87.19 &   87.03  & 
%  &       86.62    & 86.81 &  \textbf{86.91}  \\ \bottomrule

% \end{tabular}%
% }
% \end{table*}

% \begin{table*}[htbp]
% \caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) for different mechanisms under various privacy budget via sentiment analysis task over the IMDB dataset.\label{tb:2}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clccclccclccc}
% \toprule
%  &  & \multicolumn{3}{c}{\textbf{Random(seed = 42)}}           &  & \multicolumn{3}{c}{\textbf{GloVe}}                    &  & \multicolumn{3}{c}{\textbf{fastText}}                 
% \\ \cline{3-5} \cline{7-9} \cline{11-13} 
% \textbf{Privacy budget $\bm{\epsilon}$} & 
% & TrLaplace & Laplace & Guassian &  
% & TrLaplace & Laplace & Guassian &  
% & TrLaplace & Laplace & Guassian \\ \midrule
% $\bm{0.05}$  &  
% & 80.5  & 81.42 & \textbf{82.00} &  
% & 82.11 & 82.11 & \textbf{82.57}  &  
% & \textbf{82.80} & 82.00 & \textbf{82.80}  \\
% \rowcolor{lightgray}
% $\bm{0.1}$ &  
% & 81.54 & 80.62 & \textbf{82.00} & 
% & \textbf{82.34} & 82.22 & 82.22 &   
% & \textbf{82.57} & 81.88 & 82.45 \\
% $\bm{0.2}$ &   
% & \textbf{82.57} & 81.54 & 82.00 & 
% & 82.57 & \textbf{83.26} & 82.68 &  
% & 82.80 & 82.45 & \textbf{83.14}  \\
% \rowcolor{lightgray}
% $\bm{0.5}$ & 
% & \textbf{81.42} & \textbf{81.42} & 80.85 & 
% & \textbf{82.45} & 82.34 & 81.88 & 
% & \textbf{83.03} & 82.11 & 81.54  \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[htbp]
\caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) for different mechanisms under various privacy budget via sentiment analysis task over the SST-2 dataset.\label{tb:2}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clccclccclccc}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Random(seed = 42)}}           &  & \multicolumn{3}{c}{\textbf{GloVe}}                    &  & \multicolumn{3}{c}{\textbf{fastText}}                 
\\ \cline{3-5} \cline{7-9} \cline{11-13} 
\textbf{Privacy budget $\bm{\epsilon}$} & 
& TrLaplace & Laplace & Guassian & 
& TrLaplace & Laplace & Guassian & 
& TrLaplace & Laplace & Guassian \\ \midrule
$\bm{0.05}$  &  
& \textbf{86.04} & 85.97 & 84.93 &  
& \textbf{88.68} & 88.57 & 88.57 & 
& 89.37 & 89.37 & \textbf{89.40} \\
\rowcolor{lightgray}
$\bm{0.1}$ &  
& \textbf{85.44} & 84.89 & 84.06 & 
& \textbf{88.95} & 88.25 & 88.24 &   
& \textbf{89.51} & 89.50 & 89.30 \\
$\bm{0.2}$ &   
& \textbf{86.18} & 85.45 & 85.90 & 
& \textbf{88.93} & 88.51 & 88.76 &  
& \textbf{89.45} & 89.35 & 89.19 \\
\rowcolor{lightgray}
$\bm{0.5}$ & 
& \textbf{86.33} & 85.55 & 85.34 & 
& \textbf{88.88} & 88.48 & 88.60 & 
& \textbf{89.51} & 89.40 & 89.18 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> tab/tab4.tex <==
% \begin{table*}[!htbp]
% \caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) and different mechanisms under various privacy budget via sentiment analysis task in IMDB dataset.\label{tb:4}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clccclccclccc}
% \toprule
%  &  & \multicolumn{3}{c}{\textbf{Random(seed = 42)}}           &  & \multicolumn{3}{c}{\textbf{GloVe}}                    &  & \multicolumn{3}{c}{\textbf{fastText}}                 
% \\ \cline{3-5} \cline{7-9} \cline{11-13} 
% \textbf{Privacy budget $\bm{\epsilon}$}         &  & TrLaplace       & Laplace & Guassian &  & TrLaplace       & Laplace         & Guassian &  & TrLaplace       & Laplace         & Guassian \\ \midrule
% $\bm{1}$       &  & 86.78 &  \textbf{87.45} &  87.42  &  & \textbf{90.01} &      89.54     &  89.54  &  & \textbf{87.26} &     86.83      &  86.38 \\
% \rowcolor{lightgray}
% $\bm{5}$       &  & 85.96 &  \textbf{87.24} & 86.25   &  &  89.64
% & 89.81  &  \textbf{89.82}  &  & \textbf{86.59} &    86.55      &  \textbf{86.59}  \\
% $\bm{10}$       &  & 85.07 &  \textbf{87.29} & 86.31   &  & 89.82 &   \textbf{90.07}    &  89.88  & & 86.64 &   86.61        & \textbf{86.76}    \\
% \rowcolor{lightgray}
% $\bm{20}$       &  & 86.79  & 86.77  & \textbf{87.16}   &  &        89.72    & 89.70 &  \textbf{89.91}   &  &   86.65        &\textbf{86.97}  &86.40    \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

% \begin{table*}[htbp]
% \caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) and different mechanisms under various privacy budget via sentiment analysis task in IMDB dataset.\label{tb:4}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clccclccclccc}
% \toprule
%  &  & \multicolumn{3}{c}{\textbf{Random(seed = 42)}}           &  & \multicolumn{3}{c}{\textbf{GloVe}}                    &  & \multicolumn{3}{c}{\textbf{fastText}}                 
% \\ \cline{3-5} \cline{7-9} \cline{11-13} 
% \textbf{Privacy budget $\bm{\epsilon}$}         &  & TrLaplace       & Laplace & Guassian &  & TrLaplace       & Laplace         & Guassian &  & TrLaplace       & Laplace         & Guassian \\ \midrule
% $\bm{1}$ & & \textbf{82.00} & 81.31 & 81.19 &  
% & \textbf{83.26} & 83.03 & 82.57 & 
% & \textbf{82.45} & 81.77 & 82.22 \\
% \rowcolor{lightgray}
% $\bm{5}$ & & \textbf{81.42} & 81.08 & 81.08 &  
% & 82.22 & 81.77 & \textbf{82.80} & 
% & \textbf{82.22} & 81.88 & 82.00 \\
% $\bm{10}$ & & \textbf{82.00} & 80.96 & \textbf{82.00} & 
% & \textbf{82.91} & 82.45 & 82.57 & 
% & \textbf{83.60} & 82.68 & 82.91 \\
% \rowcolor{lightgray}
% $\bm{20}$ & & \textbf{82.00} & 81.31 & 81.54 & 
% & \textbf{82.34} & 81.54 & 81.54 & 
% & \textbf{83.03} & 82.45 & 82.00 \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[htbp]
\caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) and different mechanisms under various privacy budget via sentiment analysis task in SST-2 dataset.\label{tb:4}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clccclccclccc}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Random(seed = 42)}}           &  & \multicolumn{3}{c}{\textbf{GloVe}}                    &  & \multicolumn{3}{c}{\textbf{fastText}}                 
\\ \cline{3-5} \cline{7-9} \cline{11-13} 
\textbf{Privacy budget $\bm{\epsilon}$}         &  & TrLaplace       & Laplace & Guassian &  & TrLaplace       & Laplace         & Guassian &  & TrLaplace       & Laplace         & Guassian \\ \midrule
$\bm{1}$ & 
& \textbf{85.99} & 84.05 & 85.36 &  
& \textbf{89.01} & 88.61 & 88.62 & 
& \textbf{89.19} & 89.18 & 89.08 \\
\rowcolor{lightgray}
$\bm{5}$ & 
& \textbf{85.90} & 85.27 & 85.31 &  
& \textbf{88.76} & \textbf{88.76} & 88.47 & 
& \textbf{89.46} & 89.43 & 89.20 \\
$\bm{10}$ & 
& \textbf{85.27} & 84.98 & 84.57 & 
& \textbf{89.15} & 88.52 & 88.48 & 
& \textbf{89.68} & 89.45 & 89.53 \\
\rowcolor{lightgray}
$\bm{20}$ & 
& \textbf{85.75} & 85.44 & 84.12 & 
& \textbf{88.75} & 88.40 & 88.57 & 
& \textbf{89.45} & 89.40 & 89.24 \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> tab/tab5.tex <==
\begin{table}[!htbp]
\caption{Results on SST-2 data for classification task with GloVe initialization under $\epsilon=10$, where 0/1 represents the label and support is the size for each class.\label{tb:5}}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\toprule
\textbf{Mechanism} & \textbf{Label}              & \textbf{Support}               & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\ 

\hline
\rowcolor{lightgray}
Guassian  &  & & 0.87      & \textbf{0.87}  & \textbf{0.87}      \\  
\rowcolor{lightgray}
TrLaplace &      0     &        2976     & 0.88     & \textbf{0.87}   & \textbf{0.87}    \\ 
\rowcolor{lightgray}
Laplace   &                    &                       & \textbf{0.89}      & 0.84   & 0.86     \\ 

Guassian  &  & & \textbf{0.90}      & 0.90   & \textbf{0.90}     \\ 
TrLaplace &    1                &        3847         & \textbf{0.90}      & 0.91    & \textbf{0.90}     \\  
Laplace   &                    &                       & 0.88      & \textbf{0.92}   & \textbf{0.90}     \\ \bottomrule
\end{tabular}%
}
\vspace{-0.15in}
\end{table}

==> tab/utility_test.tex <==
\begin{table*}[htbp]
\caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) for different mechanisms under various privacy budget via sentiment analysis task over the SST-2 dataset.\label{tb:2}}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{Random(seed = 42)}} & \multicolumn{4}{c}{\textbf{GloVe}} & \multicolumn{4}{c}{\textbf{fastText}} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
\textbf{Privacy budget $\bm{\epsilon}$} 
& $\bm{0.01}$ & $\bm{0.1}$ & $\bm{1}$ & $\bm{10}$
& $\bm{0.01}$ & $\bm{0.1}$ & $\bm{1}$ & $\bm{10}$
& $\bm{0.01}$ & $\bm{0.1}$ & $\bm{1}$ & $\bm{10}$ \\ 

\midrule

Gaussian  &  
& \textbf{86.04} & 85.97 & 84.93 &  
& \textbf{88.68} & 88.57 & 88.57 & 
& 89.37 & 89.37 & \textbf{89.40} \\
Laplacian &  
& \textbf{85.44} & 84.89 & 84.06 & 
& \textbf{88.95} & 88.25 & 88.24 &   
& \textbf{89.51} & 89.50 & 89.30 \\
CMP &   
& \textbf{86.18} & 85.45 & 85.90 & 
& \textbf{88.93} & 88.51 & 88.76 &  
& \textbf{89.45} & 89.35 & 89.19 \\
Mahalanobis & 
& \textbf{86.33} & 85.55 & 85.34 & 
& \textbf{88.88} & 88.48 & 88.60 & 
& \textbf{89.51} & 89.40 & 89.18 \\ 
PE & 
& \textbf{86.33} & 85.55 & 85.34 & 
& \textbf{88.88} & 88.48 & 88.60 & 
& \textbf{89.51} & 89.40 & 89.18 \\ 

\midrule

Trlaplacian & 
& \textbf{86.33} & 85.55 & 85.34 & 
& \textbf{88.88} & 88.48 & 88.60 & 
& \textbf{89.51} & 89.40 & 89.18 \\ 


\bottomrule

% \vspace{-24pt}

\end{tabular}
}
\end{table*}

==> tab/utility_test_2.tex <==
\begin{table*}[htbp]
\caption{\textbf{Utility Test.} Comparison of classification accuracy with three embedding methods (Random, GloVe and fastText) for different mechanisms under various privacy budget via sentiment analysis task over the SST-2 dataset.\label{tb:2}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{Random(seed = 42)}} & \multicolumn{4}{c}{\textbf{GloVe}} & \multicolumn{4}{c}{\textbf{fastText}} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
\textbf{Privacy budget $\bm{\epsilon}$} 
& $\bm{0.01}$ & $\bm{0.1}$ & $\bm{1}$ & $\bm{10}$
& $\bm{0.01}$ & $\bm{0.1}$ & $\bm{1}$ & $\bm{10}$
& $\bm{0.01}$ & $\bm{0.1}$ & $\bm{1}$ & $\bm{10}$ \\ 

\midrule

Gaussian  &  
& \textbf{86.04} & 85.97 & 84.93 &  
& \textbf{88.68} & 88.57 & 88.57 & 
& 89.37 & 89.37 & \textbf{89.40} \\
Laplacian &  
& \textbf{85.44} & 84.89 & 84.06 & 
& \textbf{88.95} & 88.25 & 88.24 &   
& \textbf{89.51} & 89.50 & 89.30 \\
CMP &   
& \textbf{86.18} & 85.45 & 85.90 & 
& \textbf{88.93} & 88.51 & 88.76 &  
& \textbf{89.45} & 89.35 & 89.19 \\
Mahalanobis & 
& \textbf{86.33} & 85.55 & 85.34 & 
& \textbf{88.88} & 88.48 & 88.60 & 
& \textbf{89.51} & 89.40 & 89.18 \\ 
PE & 
& \textbf{86.33} & 85.55 & 85.34 & 
& \textbf{88.88} & 88.48 & 88.60 & 
& \textbf{89.51} & 89.40 & 89.18 \\ 

\midrule

Trlaplacian & 
& \textbf{86.33} & 85.55 & 85.34 & 
& \textbf{88.88} & 88.48 & 88.60 & 
& \textbf{89.51} & 89.40 & 89.18 \\ 

\bottomrule

\end{tabular}%
}
\end{table*}
